Two-dimensional inference of divertor plasma characteristics: advancements to a multi-instrument Bayesian analysis system

An integrated data analysis system based on Bayesian inference has been developed for application to data from multiple diagnostics over the two-dimensional cross-section of tokamak divertors. Tests of the divertor multi-instrument Bayesian analysis system (D-MIBAS) on a synthetic data set (including realistic experimental uncertainties) generated from SOLPS-ITER predictions of the MAST-U divertor have been performed. The resulting inference was within 6\%, 5\% and 30\% median absolute percentage error of the SOLPS-predicted electron temperature, electron density and neutral atomic hydrogen density, respectively, across a two-dimensional poloidal cross-section of the MAST-U Super-X outer divertor. To accommodate molecular contributions to Balmer emission, an advanced emission model has been developed which is shown to be crucial for inference accuracy. Our D-MIBAS system utilises a mesh aligned to poloidal magnetic flux-surfaces, throughout the divertor, with plasma parameters assigned to each mesh vertex and collectively considered in the inference. This allowed comprehensive forward models to multiple diagnostics and the inclusion of expected physics. This is shown to be important for inference precision when including molecular contributions to Balmer emission. These developments pave the way for accurate two-dimensional electron temperature, electron density and neutral atomic hydrogen density inferences for MAST-U divertor experimental data for the first time.

==> Bin.tex <==
%%%%%%%%%%% INTRODUCTION %%%%%%%%%%%%%%%%%%%%%%%%
% priors that can be naturally incorporated to the IDA by aligning the grid to surfaces of constant magnetic flux enable the IDA to accurately infer the underlying plasma parameters with forward models that include PMI. We lay out the steps required to accommodate the PMI's inclusion in the Balmer line forward models of the IDA. We consider the impact of including helium within the inference and the increase in inference accuracy of utilising the priors enabled by the new grid. Finally, we utilise the synthetic data to consider how well the IDA can reflect the error as uncertainty within the inference.

% % Our proposed solution
% Additional diagnostics, not subject to PMI, are available to the IDA such as Helium emission lines (). However, these too come with additional parameters to be included within the inference. The growing parameter space poses a challenge to the IDA's ability to accurately infer the plasma parameters. % does this need explaining?
% To reduce the size and complexity of this vast parameter space, pre-conceived knowledge of the plausible regions of parameter combinations can be injected into the IDA (the \textit{priors} of Bayesian inference). Much of the physics associated with charged species in the divertor are tied to surfaces of constant poloidal magnetic flux.  % this last bit should be re-worded
% Consequently it follows that the inclusion of physics-based priors ought to heed these flux surfaces.



%%%%%%%%%%% Background %%%%%%%%%%%%%%%%%%%%%%%%

% When to combine the data-sets in integrated data analysis is not obvious. Taking raw data from each diagnostic often requires many parameters to be included in the forward models. Processing the data first allows simpler forward models in the inference but risks \textit{loosing} information from the data through simplifications in the processing. An example pertinent to this work is in the inversion of camera images (see sec). Camera data could be `inverted' in an attempt to find the emissivity coming from a single point in the plasma. However, this inversion depends on other emissivities throughout the plasma; one region of plasma immediately in-front of the camera might be known by another diagnostic to be strongly emitting and consequently the emissivity contribution from other regions of the plasma would be reduced. However, by `pre-inverting' the data, each plasma region is treated independently and consequently information is lost. Consequently, work using such `cell-based' inference as performed by (Artur, Tijs) requires substantial error regions and is therefore not suitable for accurate inference of the Te, ne and n0 fields.

% The collective treatment of plasma parameters throughout the divertor region was shown to work in \cite{Bowman_2020} IDA. This `mesh-based' inference evaluated electron temperature, electron density and neutral density at mesh vertices spread over a poloidal cross section generating a large vector of inference parameters. This vector of parameters was subsequently used to model the camera brightness images themselves rather than the pre-inverted data. It also allowed for other diagnostics such as Thomson Scattering and Langmuir probes to be included in the inference. 

% The IDA outlined in (Chris) inverted the labour-intensive process of fine-tuning modelling codes, such as SOLPS-ITER, to match data observed in experiment by available diagnostic systems. The plasma state (electron temperature, electron density and neutral density at various spatial points within the divertor) formed the vector of inference parameters, $\thetavec$, and the probability of each plasma state given the measured diagnostic data set, $\mathcal{D}$, was calculated. This `posterior' probability was found through Bayes' theorem,
% \begin{equation}
%     \underbrace{P(\theta|\mathcal{D})}_{\mathrm{posterior}} \propto  \underbrace{P(\mathcal{D}|\theta)}_{\mathrm{likelihood}}\times \underbrace{P(\theta)}_{\mathrm{prior}}.
%     \label{eqn:bayes}
% \end{equation}
% The prior probability of equation~\ref{eqn:bayes} represents pre-conceived knowledge in the plausibility of a plasma state. These may be spatially independent, such as a maximum expected electron temperature, and as such can be used in either cell- or mesh-based inference. A key benefit to the mesh-based inference outlined in \cite{Bowman_2020} is the ability to include spatially dependent prior information, namely, the expected `smoothness' of each plasma field. The cost of such inference is the requirement to jointly consider \etemp, \edens\, and \ndens at many spatial locations (forming an `inference mesh') throughout the divertor region. 

% Why is HMC and NUTS required
% The mesh-based method's large number of dimensions requires, unlike the cell-based method, the Hamiltonian Monte Carlo (HMC) sampling method \cite{neal2011mcmc} to efficiently characterise the posterior distribution. The No-u-turn (NUTS) sampling method \cite{hoffman2014no} advances HMC by automating the selection of number of steps conducted by the Hamiltonian simulation; this is paramount for sampler to aptly explore the full distribution and collate a set of samples that fairly reflects the posterior distribution. Considerable computational power is required for such sampling methods in high dimensions and a smooth, differentiable posterior distribution is required. This removes the possibility of mesh-based inference to use non-differentiable priors and be conducted inter-shot () - both of which are permitted by the cell-based inference.

% This results in the requirement of thousands of parameters to be in the inference. Advanced optimisation methods are required to find the plasma state at highest posterior probability (maximum a posteriori, MAP) as outlined in appendix A of Chris and computationally-expensive methods such as Markov Chain Monte Carlo are required to adequately sample the high-dimensional parameter space. Thus, for tractable solutions, only smooth, differentiable prior probability distribution can be included in the inference. These problems dissipate when undergoing `cell' based inference as is performed in (). Here, inference is individually carried out at discrete spatial locations in the divertor and so the parameter vector is only comprised of a single value for \etemp, \edens\, and \ndens. However, this cell-based inference cannot include the spatially dependent priors that we find to be necessary for inference with advanced forward models.

% \subsection{Equilibrium Reconstruction}
% % The grid and equilibirium reconstruction
% Grid points are chosen to follow flux surfaces as shown in Figure (). Owing to limited plasma current in the divertor chamber, the equilibirum reconstruction is predominantly governed by coil currents. This reduces uncertainty in the reconstruction. 




%%%%%%%%%%% Method %%%%%%%%%%%%%%%%%%%%%%%%


% The result is $N$ mesh vertices, $(j=0,...,j=N)$. 
% Within $\mathbb{J}$ are: () subsets of grid points parallel to flux surfaces at $\psi=()$, $\mathbb{J}_{\parallel, \psi}$; and () subsets of grid points perpendicular to flux surfaces at an average distance of () to the target, $\mathbb{J}_{\perp, s}$.



When faced with data that appears to contradict the priors, a reasonable difference between the prior argument and the expected value must be permitted. As such, a multivariate Gaussian probability distribution is applied on each prior (where each dimension corresponds to a point at which the prior is analysed). For a prior, $_i$, with difference between the argument, $\xvec_i=\left(x_0,...,x_{N_i}\right)$, and expected, $\muvec_i\left(\mu_0,...,\mu_{N_i}\right)$ of $\Deltavec_i$,
\begin{equation}
    \mathcal{L}(\thetavec)_i = \left(-\frac{1}{2}\sigma_i^{-2}\Deltavec_i^T\Deltavec_i- \log\left(\sigma_i\right) - \frac{N_i}{2}\ln(2\pi) 
 \right)
\end{equation}

We analysed the suitability of Gaussian and Cauchy probability distributions in the priors. It was found that smoothing was more suitable in ().


Through $\Deltavec$, the size of $\log(Prior)$ depends on discretionary aspects such as units and the number of points at which the prior is analysed ($N_i$, typically the number of grid points). Furthermore, for some priors, such as the smoothing priors, the true solution does not lie at the maximum prior probability. Consequently, each prior's probability must be adapted to avoid \textit{over-enforcement} (where the prior probability benefit of solutions adhering to the prior usurps the likelihood penalty of ignoring the data) and \textit{under-enforcement} (where solutions over-fit the data since there is not enough of a prior probability penalty for significantly breaching the prior) of the prior. To handle this, two approaches were considered and contrasted: scaling the uncertainty and standardising $\Delta$.

\subsubsection{Scaling the uncertainty}
The uncertainty for each of the . Since the effects of each prior cannot be individually isolated, a multi-dimensional scan was required. The $T_e$ and $n_e$ parallel smoothing uncertainties were considered to be similar as were the $n_0$ parallel and perpendicular uncertainties. The results of the scan are shown in Figure (). For ease, try to compress this into a collection of 1 d scans. For brevity, the MAP was sought rather than MEX.
\begin{figure}
    \centering
    % \includegraphics{}
    \caption{Figure to show MAPE for multiple solps cases and for each of the uncertainties individually }
    \label{fig:my_label}
\end{figure}

The deficiencies of this method are that the scan would need to be repeated for each grid (e.g smoothing uncertainties may alter for super-x versus conventional divertor configurations) and cannot easily be updated with new data.



\subsubsection{Standardising Delta}
 The standardisation of $\Deltavec$ (b) was performed by $\Deltavec\to \Deltavec/\left\langle\sigma_{\Delta}\right\rangle_{solps}$. For priors that were single sided, the standard deviation of the mirrored result was used. A benefit of (b) is that the catalogue of cases contributing to $\langle\Deltavec^T\Deltavec\rangle$ can be updated with real data once the IDA is being reliably performed. The uncertainty of each prior, $\sigma$, can be left as a free parameter. As shown in Figure (), by setting a lower and upper limit on $\sigma$ of $\sigma^l$ and $\sigma^u$ respectively, $\log(P_i)$ decreases () until $\left|\Deltavec\right|=\sigma^l$...  $\sigma^l$ needs to be large enough so not to \textit{over-enforce} the prior by significantly preferring solutions of low $\Deltavecsquared$. $\sigma_u$ needs to be low enough so not to \textit{under-enforce} the prior by permitting large $\Deltavecsquared$ without significant probability penalty. The normalisation of $\Deltavecsquared$ enables a sensible range of ($\sigma^l$, $\sigma^u$) of (0.2, 5) common to all priors. To ensure that the posterior probability acts to prevent an over-fit to the data, the overall prior probability, may be scaled such that,
\begin{equation}
    \log(Prior) = A\sum_{i}\log(Prior_i).
\end{equation}
A scan across many values of A for multiple test cases (shown in Figure) found () to be optimal. This corresponds to each prior having incentive to overrule the increased posterior probability of $\thetavec_{MLE}$ over $\thetavec_{true}$ which is performed when 
\begin{equation}
    \left\langle \log\frac{P(\thetavec_{MLE})}{P(\thetavec_{true})}\right\rangle\approx A\log\frac{\sigma^l}{\sigma^u}.
\end{equation}


solutions are not usurped To ensure any prior does not usurp In the face of conflicting 
To ensure the prior does not absolutely refuse solutions presenting a prior argument different to the expected value in the face of conflicting data,. For example  a Gaussian  prior is considered


However, owing to the fact that there is no two-dimensional poloidal cross section data for our parameters (which itself is the very motivation of the IDA) priors based on sound, physical theory are required. Computational models can be used to check these priors, however since the same physical theories are typically embedded into the models an over-dependence on these models risks biasing the IDA outputs. Therefore, whilst these priors can initially lean on the models to get reasonable results, they must be written in such a way to be easily updated once experimental data is available, such that the IDA continuously \textit{learns}. As such, three facets are required: a normalisation term for each prior that can be routinely updated once more data becomes available; a flexible prior uncertainty; a single scaling term that can be applied to the prior probabilities

\subsubsection{Prior Method Comparison}
For comparison of the `scanned sigma' and `learned sigma' approaches to handling the priors, a one dimensional test case was utilised. A function, $f(\psi; \alpha)$, was chosen to reflect example temperature profiles (perpendicular to surfaces of constant poloidal flux) for a set of scenarios, $\alpha \in A$, (such as degree of detachment, up-stream pressure and distance to target). The parameters in the inference, $\thetavec$, were these temperature values evaluated at positions where a diagnostic exist, $\thetavec_M$, and positions where no diagnostic exists, $\thetavec_{M'}$, such that $\thetavec = (\thetavec_M, \thetavec_{M'})$. For each $f(\psi; \alpha)$, N synthetic data sets were produced for the M measurement positions each with a Gaussian error of $\sigma_{noise}$ applied, $D(\psivec_M; n, \alpha)$, where $n\in N$. For the inference, a Gaussian likelihood was applied at each measurement location and a Gaussian prior was applied to the second derivative for each element of $\thetavec$. The log-likelihood is therefore given by, 
\begin{equation}
    \mathcal{L}_{like}\left(D|\thetavec\right) = -\frac{1}{2}\sum_i\left(\frac{\theta^{(i)}-D^{(i)}}{\sigma_{noise}}\right)^2.
\end{equation}
For the `scanned sigma' case, the log-prior is given by,

\begin{equation}
    \mathcal{L}_{scan}\left(\thetavec|\sigma\right) = -\frac{1}{2}\sum_j\left(\frac{\Delta^{(j)}}{\sigma}\right)^2,
\end{equation}
where $\Delta^{(j)}$ is the j-th element of $\frac{\partial\thetavec}{\partial\psi}$. For the `learned sigma' case, the log-prior is given by,

\begin{equation}
    \mathcal{L}_{scan}\left(\thetavec, \sigma\right) = S\left(-\frac{1}{2}\sum_j\left(\frac{\tilde{\Delta}^{(j)}}{\sigma}\right)^2 - \log(\sigma)\right).
\end{equation}

where $\tilde{\Delta}^{(j)} = \Delta^{(j)} / \left(N\langle\rangle\right)$ . Such standardisation ensures that (everything is kept within the graph range) and consequently sensible limits can be put on $\sigma$. The scale factor, S, manages the demand for the smoother, true solutions ($\thetavec_{true}$) to be chosen over the noisier, maximum-likelihood estimate ($\thetavec_{MLE}$) solutions that over-fit to the data. The average log-likelihood difference between the two must therefore be matched to the log-prior difference between choosing $\sigma_l$ over $\sigma_u$ such that,
\begin{equation}
    S = \frac{\langle \mathcal{L}_{like}\left(D|\thetavec_{MLE}\right) - \mathcal{L}_{like}\left(D|\thetavec_{true}\right) \rangle}{\log(\sigma_u) - \log\left(\sigma_l\right)}.
\end{equation}

For the scanned sigma approach, across the different data-sets it was found that the different $\alpha$ cases had different optimal $\sigma$ values. Therefore, for when the true solution is unknown, a single, optimal $\sigma$ value could not be pre-determined. Consequently there is risk of artificially over or under-enforcing the priors. As shown in Figure (), averaged across the data-set, the `learned sigma' approach performs better than any one $\sigma$ from the scan. Further investigation showed that the found sigma in each case was within () of the sigma that maximises () of equation (). For the `learned sigma' approach, a representative data set is required to find $S$ and $N\langle\rangle$. To observe sensitivity to these values, validation cases were generated to be both within () and outside () of the $\alpha$ parameters used to create the training set. It was found that the `learned sigma' approach managed to handle these validation cases. Consequently, this method was adopted moving forward. 
% How does this relate to the errors? 


% \paragraph{Normalisation Term}
% The probability associated with each Gaussian prior is a function of the separation between the nominal, expected result of the \textit{prior} function, $\muvec$ and the prior function's result based on the parameters, $\xvec=f(\thetavec)$. To remove the dependence of the size of this separation, $\Deltavec = \xvec-\muvec$, on scaling factors in the prior function (eg. choice of unit system), it is to be written as a fraction of the average result of the prior function based on data available. It is this data that must initially depend on models but will transition to depend on experimental data, based on previous IDA runs, as the IDA \textit{learns}. Consequently,
% \begin{equation}
%     \Deltavec^T\Deltavec \to \frac{\Deltavec^T\Deltavec}{N\langle \overline{\Deltavec^T\Deltavec}\rangle_{data}}
% \end{equation}


% \paragraph{Prior Uncertainties}
% Since the prior function's are simply based on ideal physics theory, the question of how much uncertainty to apply to the prior's probability is ambiguous. How much lower should the probability of a parameter set that slightly breaches the prior function's condition be in comparison to one that drastically violates the prior's limits? This is controlled by the prior's uncertainty (the Gaussian $\sigma$). To allow for slight errors in the equilibrium reconstruction (of which the priors are sensitive to) and for cases that unexpectedly decisively disagree with a prior, we suggest letting the IDA \textit{learn} the prior uncertainty which in turn dictates how strongly the prior should be enforced. This is 

% \paragraph{Scaling Term}
% The . The normalisation of each prior removes the arduous need to find a scaling term for each prior and allows a single scaling term to be applied across all priors collectively.


% What is important here is that we want to write the priors in such a way that we have a single parameter to scan



% Whilst it may be possible to conceive a physics basis for why a prior may be implemented, the question of the associated probability of solutions that breach the prior's limits is considerably more ambiguous. It is reasonable to suppose that a solution that slightly breaches a prior is more probable than one that dramatically breaches the prior. The question of how quickly a prior's probability tends to zero once it has been breached corresponds to the \textit{uncertainty} in the prior.

% This question is easy to answer once experimental data for the desired parameters is available: the prior uncertainties can be updated to correspond with the distribution of results. In the absence of experimental data, it is unwise to depend too heavily on models since these typically also impose the same physics basis that we desire in our priors and as such would bias results. To counter this, the uncertainty of each prior is left as a hyper-parameter to the problem with the IDA left to \textit{learn} how strongly each prior should be imposed. This is performed through normalisation.

% The priors used were applied over the difference between a function of the parameters, $\xvec=f(\thetavec)$, and the expected output of this function, $\muvec$. The difference in these, $\Deltavec = \xvec - \muvec$, has N elements and so results in an N-dimensional, multivariate Gaussian prior. The covariance matrix of this prior is taken as $\sigma^2 I_N$. Thus,

% The same prior is commonly applied numerous times
% \begin{equation}
%     \log(P) = \left(-\frac{1}{2}\sigma^{-2}\Deltavec^T\Deltavec- \log\left(\sigma\right) - \frac{N}{2}\ln(2\pi) 
%  \right)
% \end{equation}

% Consider imposing a prior over a function of our parameters. Imposing the Gaussian prior results in a multivariate Gaussian distribution of dimensionality of the number of times the prior is enforced.  prior over parameters $\alphavec\subseteq\thetavec$. The result is a multivariate 



% The impact of such a normalisation scheme is shown in Figure (). In (ai) the normalised delta at which 68\% of the vector elements are contained is shown for the solps results. In (aii) the same result is shown but for maximum likelihood inferences based on the same solps results. 

% \subsubsection{Uncertainty Strength Comparison}
% Do the one dimensional example here



% Assuming the availability of spatial \etemp\, and \edens\, measurements from both Langmuir probe (LP) and Thomson scattering (TS) diagnostics (though, the raw measurements can be modelled from \etemp\, and \edens, $f_i(\theta)$ of~(\ref{eqn:Likelihood}) need simply extract a vector of \etemp\, and \edens\, from Eq.~\ref{eqn:parameter_vector}. $W_i$ carries pre-calculated linear interpolation weights that specify each mesh vertices' contribution to the diagnostic measurement's spatial location. $\mathbf{\Sigma}$ was chosen to carry a single uncertainty, $\sigma$, with no correlations between measurements such that $\sigma_{\text{D, F}}^2 \mathbf{I}$ for D$\in$ \{LP, TS\} and F$\in$\{\etemp\, and \edens\}.

% For the MWI, Balmer lines \{3($\alpha$),...,7($\epsilon$)\}$\to$ 2 and Helium lines \{502nm, 668nm, 728nm\} were chosen. The measured quantity is the brightness of each camera pixel so, for these forward models, $f_i(\theta)$ was the calculated the emissivity, $\varepsilon$, of a line which. For the Balmer lines $\varepsilon$ is given by Eq.~\ref{eqn:Balmer_emissivity} and for the Helium lines, $\varepsilon$ is given by Eq.~\ref{eqn:emissivity} where $i\in$\{recombination, excitation\} with densities (\edens, \nhepdens) and (\edens, \nhendens) respectively. For filtered camera images, $\mathbf{W}$ takes the emissivities at each vertex and casts them to a vector of pixel brightnesses. The camera diagnostic's covariance matrix $\mathbf{\Sigma}$ and are taken to be uncorrelated between different cameras and of the form given by Eq.~11 of \cite{Bowman_2020}. 

% The full parameter set is therefore,
% \begin{equation}
%     F = \left\{T_e, n_e, n_0, Q_{mol.}, n_{He^0}, n_{He^{1+}}\right\}.
% \end{equation}



% \subsubsection{Spatially-Independent Priors}
% We consider `spatially-independent priors' to be those that have no information about parameter values at a different mesh vertex. These can be applied by any inference mesh or cell based method. These include the expected ranges of each of the parameters. They also include priors that consider the interplay of each parameter at each grid vertex, for example the static pressure and neutral fraction priors of \cite{Bowman_2020}. For the neutral and singly charged helium, we consider limits on the permitted range of $\left(n_{He_0}+n_{He_1}\right)/n_e$ and $n_{He_1}/n_{He_0}$ (dubbed `helium concentration ratio' and `ionisation ratio' respectively since Helium 2+ plays no significant role in our analysis). We also utilise available SOLPS-ITER simulations to investigate the expected ranges of $n_{He_0}$, $n_{He_1}$ and $Q_{mol.}$. Consideration of the Balmer line emission of equation () outlines how, in regions of high temperatures, slight under-estimation of $n_0$ permits the excitation contribution to be replaced by molecular contribution. Consequently, a minimum limit is placed on the neutral fraction, $n_{0}/\left(n_{e}+n_{0}\right)$, based on expected values from SOLPS-ITER simulations.

% \subsubsection{Spatially-Dependent Priors}
% Spatially-dependent priors are those for which the prior at one vertex is calculated using information of parameter values at a different vertex. These are not possible in the cell-base method. Since the priors suggested below are linked to flux surfaces, we claim them to be `field-aligned-mesh-enabled' (they could be deployed using any mesh, however at a significant computational cost since interpolation between two mesh vertices would be required to find the field values on a flux surface).



% The collective treatment of all parameters at each grid vertex permits priors related to parameter relationships between grid points. This includes how much a parameter is expected to vary between grid points (it's `smoothness') as was demonstrated in (Chris). Whilst the following priors plausibly can be applied on any grid, they become computationally feasible when applied to grid vertices pre-arranged to follow surfaces of constant poloidal magnetic flux. Unlike the standard priors, it is plausible (and often expected) that these priors will be breached: a more smooth solution is considered more realistic but we do not expect perfectly smooth solutions. Consequently, how strongly to impose each of these grid-enabled priors needs to be carefully considered. The scheme we suggest is (to let the IDA learn how to strongly impose the prior). Explain the prior handling methodology in an appendix. 


% Why priors?: This could be moved to the introduction
% The role of a prior is to inject preconceived knowledge into the problem. This offers an extremely powerful tool in a regime where diagnostic coverage is limited; they are able to restrict the need for our optimisation and sampling algorithms to explore substantial regions of parameter space. Consequently, considered use of priors means that more complex models (accompanied by additional parameters) become computationally conceivable. 

% The overall prior consists of the product of multiple priors which have been chosen based on expected physical theory that have been observed in experiments (reference). These include: .

% Those priors that are easily enacted irrespective of the grid are: 



% \subsubsection{Prior probability distributions}
% Outline standard, empirical and full Bayes

% An important aspect of the priors outlined in Tables \ref{tab:grid-enabled priors}
% Some of the priors may be well characterised by a Heaviside step function style distribution; the probability is constant up until the prior is `breached' after which the probability drops to zero. However, many priors are expected to be breached. Consequently, we would expect a plasma state with smooth fields to be more probable than a plasma state with rapidly fluctuating fields however it would be wrong to reject anything other than plasma states with perfectly smooth fields since then only flat fields would be permitted. Consequently, the probability distribution that a prior follows needs to be carefully considered.

% Each prior argument, $x_i^k$, was taken to be from a single distribution representing prior $i$. For insight into these distributions, each prior argument was evaluated at each mesh vertex for all available SOLPS-ITER simulations (excluding those used to create the synthetic data in this analysis, see section ()). Figure \ref{fig:prior_hist} shows a representitive distribution of the prior argument (). It was found that for all priors outlined in \ref{tab:grid-enabled priors} and \ref{tab:standard priors}, the heavy-tailed Cauchy distribution best characterises the distribution. This was due to the distribution recognising that their may still be extreme breaches of the prior (such as a sharp kink in electron density close to the target) despite the vast majority of values either not breaching or minimally breaching the prior. The scale of the Cauchy distribution, $\gamma$,  was taken empirically as one half of the inter-quartile range of the prior argument applied to all available SOLPS-ITER datasets.

% The resultant log-probability of prior $i$, evaluated at mesh vertex $k$, is therefore taken as,
% \begin{equation}
%     \mathcal{L}_i(x_k) \propto \log(\gamma_i) - \log\left(\left(x_i^k\right)^2 + \gamma_i^2\right).
% \end{equation}

% Simplifying the posterior distribution is beneficial for relaxing computational cost and due to Occam's razor. This paper has introduced three components to the posterior distribution: the molecular emission model of equations \ref{eqn:alpha_mol_emission} and \ref{eqn:Balmer_emissivity} (demanding the additional field parameter $Q_{mol.}$); the spatially-dependent priors (outlined in table \ref{tab:grid-enabled priors}); and the MWI helium line data (demanding additional field parameters $He_0$ and $He_1$). 


% \begin{table*}[]
%     \centering
%     % \begin{tabular}{p{5cm}p{5cm}lp{6cm}}
%     \begin{tabular}{ccccccc}
%     \toprule
%          & \multicolumn{4}{c}{Likelihood} & \multicolumn{2}{c}{Prior} \\
%          &   & \multicolumn{2}{c}{Balmer MWI} &   &   &   \\
%          & TS+LP & Atomic Model & Molec. Model & Helium MWI & Spatially-dependent & Spatially-independent \\
%      \midrule
%      Posterior A & \checkmark  & \xmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark \\
%      Posterior B & \checkmark  & \checkmark  & \xmark  & \checkmark  & \checkmark  & \checkmark \\
%      Posterior C & \checkmark  & \xmark  & \checkmark  & \checkmark  & \xmark  & \checkmark \\
%      Posterior D & \checkmark  & \xmark  & \checkmark  & \xmark  & \checkmark  & \checkmark \\
%      \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:posterior_distributions}
% \end{table*}

% \subsection{Comparison Metric}
% The use of synthetic data permits a comparison between the true plasma fields and the inferred fields. For succinct comparison, the comparison metric was chosen to be the mean absolute percentage error (MAPE) between the true and inferred values of each plasma field $f^k\in \{T_e, n_e, n_0\}\subseteq\thetavec$ at each mesh vertex considered to contribute at least 1\% of the total emission recorded by the MWI ($k\in \{j=0,...,j=N\}$). The comparison metric is therefore given by
% \begin{equation}
%     MAPE = \frac{1}{3N_k}\sum_{f^k\in\{T_e, n_e, n_0\}}\sum_{k}^{N_k} \frac{\left|f_k^{infer}-f_k^{true}\right|}{f_k^{true}}\times 100\%.
% \end{equation}

% The true values, $\thetavec$, were those taken from SOLPS-ITER simulations to produce the synthetic data. It is worth noting that since error, replicating, was applied to each diagnostic measurement, there is always expected to be a difference between $\thetavec_{true}$ and $\thetavec_{infer}$. $\thetavec_{infer}$ may be interpreted as ($\theta_{MAP}$ and $\theta_{MEX}$).

% We further note the importance of being able to extract uncertainties from the posterior distribution. The complexity of our distribution meant that the computational expense of ensuring the HMC Markov chains were run to a stationary state could not be achieved and consequently could lead to issues in the uncertainty estimation. To each posterior, we attribute a score, $N_5$, that is the percentage of parameters that contain the true value within it's estimated 95\% confidence interval. An $N_5$ score of above or below 95\% respectively suggest an over- or under-estimation of the uncertainty. 


% \subsubsection{Molecular Density Post-Processing}
% SOLPS-ITER provides information on molecular density of (), and so for its molecular contribution,  . For comparison purposes, Q-mol was also extracted via ().




%%%%%%%%%%% Results %%%%%%%%%%%%%%%%%%%%%%%%

% The neutral density was less successfully inferred, however the posterior distribution was able to place the true values within the 95\% confidence interval for 94\% of \ndens{}\, parameters. This is indicative of an inherent uncertainty in \ndens{} due to its limited influence in equation \ref{eqn:Balmer_emissivity}. The 



% \subsection{Comparison}
% % Comparison to MLE case
% Figure () shows that the usage of priors, enabled by a grid aligned to flux surfaces, results in a mean absolute percentage uncertainty far exceeding the MLE across all test cases.

% The figure shows the grid with no helium and no GA priors (analogous to the previous case), the grid without helium but with GA priors, the grid with helium and no GA priors, the grid with helium and GA priors. Do this for both helium cases available. What was found is that the electron temperature and neutral density were regularly being under-predicted. This was enabled by the excitation emission being replaced by molecular emission. The inclusion of helium reduces this under-prediction of the temperature since the helium camera images could not be matched without a raised temperature. The inclusion of the GA priors helped in two ways: firstly, it reduced over-fitting to what we know to be noisy data; secondly, the camera inversion.

% with the camera inversion: with the MWI's inverted image, camera brightness could have occurred from variuous places. By using the priors, we know 


\begin{figure}
    \centering
    \includegraphics[width=.5\linewidth]{Figures/Percentage_Comparison.png}
    \caption{Percentage Comparison, add various solps files here. Add MEX. Add previous grid implementation.}
    \label{fig:Percentage_Comparison}
\end{figure}

% \subsection{Helium Inclusion}
% What are the results of the old grid but with Helium inclusion? The old grid should simply have priors that do not depend on field lines:


% What if Helium is not included? The priors are not enough: the role of PMI is significantly over-estimated upstream






\subsection{Prior Scans}
Observe which prior result was best - should this be in the method section?

\subsection{Inference}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/Field Comparison (MAP).png}
    \caption{Field Comparison. Is it better to do this for the MEX?.
    }
    \label{fig:Field Comparison}
\end{figure}

\subsection{Sampling Check}
% Comparison of sampled uncertainty to the true error
Figure () contrasts the estimated 95\% confidence interval, from Hamilitonian MCMC sampling, compared to the true error.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/MEX Scatter.png}
    \caption{MEX Scatter. Restricted to analysis points at which there is a minimum of 1\% contribution to the error. The number of true data points lying within the 95\% confidence interval of the MEX are 85\%, 91\% and 79\% for the Te, ne and n0 respectivley.
    Note this has just been performed for the seed 2 case: should be repeated for multiple solps files.
    }
    \label{fig:MEX Scatter}
\end{figure}


Derived fields (ionisation fraction etc.)
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/Derived Parameters.png}
    \caption{Derived Parameters}
    \label{fig:Derived Parameters}
\end{figure}

% Could we tackle the calibration here?
Analyse the impact of having the calibration included




% \subsection{Sampling Check}
% Critical to use on experimental data is a robust procedure to find the uncertainty of the inference.


% % Comparison of sampled uncertainty to the true error
% Figure () contrasts the estimated 95\% confidence interval, from Hamilitonian MCMC sampling, compared to the true error. X points contained the true value within it's 95\% confidence interval indicating that the sampling was ().


% \begin{figure*}[!ht]
%     % \captionstyle{centerlast}
%     \begin{minipage}[l]{1.0\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Figures/MEX Scatter.png}
%     \end{minipage}
%     \hfill{}
%     \begin{minipage}[r]{1.0\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Figures/MEX Scatter.png}
%     \end{minipage}
%     \caption{MEX Scatter. Restricted to analysis points at which there is a minimum of 1\% contribution to the error. The number of true data points lying within the 95\% confidence interval of the MEX are 85\%, 91\% and 79\% for the Te, ne and n0 respectively.
%     Note this has just been performed for the seed 2 case: should be repeated for multiple solps files.
%     }
%     \label{fig:MEX Scatter}
% \end{figure*}

% \begin{figure*}[!h]
%     \centering
%      \begin{subfigure}
%         \includegraphics[width=\linewidth]{Figures/MEX Scatter.png}
%      \end{subfigure}
%      \begin{subfigure}
%     \includegraphics[width=\linewidth]{Figures/MEX Scatter.png}
%      \end{subfigure}
%     \caption{MEX Scatter. Restricted to analysis points at which there is a minimum of 1\% contribution to the error. The number of true data points lying within the 95\% confidence interval of the MEX are 85\%, 91\% and 79\% for the Te, ne and n0 respectively.
%     Note this has just been performed for the seed 2 case: should be repeated for multiple solps files.
%     }
%     \label{fig:MEX Scatter}
% \end{figure*}


% Could we tackle the calibration here?
% Analyse the impact of having the calibration included




%%%%%%%%%%% Discussion %%%%%%%%%%%%%%%%%%%%%%%%

==> Theory.tex <==
\section{Background}
\subsection{The MAST-U Divertor}
% Discuss the available diagnostics, their benefits and limitations
Multiple diagnostics in the MAST-U lower, outer divertor region give insight into the electron temperature and electron density. Those diagnostics that can be accurately modelled with minimal additional parameters are of most use to the IDA. Two such diagnostics are MAST-U's divertor Langmuir probe and Thomson scattering systems for which \cite{Fevrier2018LP} and \cite{Hawke_2013TS} respectively demonstrate that \etemp{} and \edens{} measurements at discrete spatial locations can be extracted from raw data. 

The multi-wavelength imaging system (MWI) provides filtered camera images of atomic transitions \cite{mwi}. The emissivity of a specie's atomic transition $m\to n$ (at a spatial location) can be modelled via,
\begin{equation}
\varepsilon^{m\to n} = \sum_i n_{i, 0} n_{i, 1} PEC^{m\to n}_{i}(T_e, n_e),
\label{eqn:emissivity}
\end{equation}

where $i$ is a contributing process to that emission which in turn depends on the densities of the two species involved, $n_{i, 0}, n_{i, 1}$, in the process and the photo emissivity coefficient, PEC, of the process typically provided by ADAS \cite{adas}.
The hydrogenic Balmer line and helium singlet line emission are typically modelled through two predominant, atomic processes: electron-impact recombination (EIR) and electron-impact excitation (EIE). 
% This allows emission from these lines to be parameterised by just: \etemp, \edens; \ndens, \nhpdens (which assuming a plasma effective charge of 1 is equated to \ndens) for Balmer lines; and \nhendens, \nhepdens for Helium lines.
% Why are we looking at the Super-X divertor and what are the impacts of this
However, \cite{Verhaegh_2022} has shown that in MAST-U's Super-X divertor,
% enacts total magnetic flux expansion in the divertor region which has been shown through models (\cite{Fil_2022}) to reduce heat and particle fluxes to the divertor walls. 
hydrogen molecules play an important role in the plasma dynamics through molecular activated recombination (MAR) and molecular activated dissociation (MAD). MAR and MAD create excited hydrogen atoms and so PMR must be considered as an additional process in Eq.~\ref{eqn:emissivity}.

\subsection{Integrated Data Analysis}
% How does Bayesian inference work
Bayesian inference hypothesises that data from each diagnostic, $\mathcal{D}$, are fundamentally true and forward models predict this data set from model parameters, $\theta$. The \textit{posterior} probability of a certain model parameter combinations given this data is given by,
\begin{equation}
    \underbrace{P(\theta|\mathcal{D})}_{\mathrm{posterior}} \propto  \underbrace{P(\mathcal{D}|\theta)}_{\mathrm{likelihood}}\times \underbrace{P(\theta)}_{\mathrm{prior}}.
    \label{eqn:bayes}
\end{equation}
The many different parameter combinations result in a posterior distribution of which the maximum a posteriori probability (MAP) can be claimed as the inferred $\theta$ and sampling from the distribution can provide the uncertainty on this inference. The number of parameters in $\theta$ dictates the dimensionality of the distribution and complex procedures are required to ensure faithful sampling of the potentially vast, multi-modal posterior distribution as outlined in \cite{neal2011mcmc, hoffman2014no}. 

% Why analyse on a mesh
The MWI cameras offer a tangential view of the plasma, whereas profiles on poloidal cross sections are more desirable for interpretation. Consequently, the camera image data requires inverting to find the emissivity arising from each point in the poloidal cross-section for a full MWI forward model. `Cell-based' inference pre-inverts camera data into multiple independent data contributions from discrete spatial locations in the poloidal cross section, \textit{cells}, such that many smaller inference problems can be performed \cite{Perek_2022}. This reduces the total number of model parameters making the posterior distribution easier to acquire. However, \cite{Bowman_2020} demonstrated that the additional information held by not pre-inverting the MWI data and jointly considering parameters distributed over a mesh across a poloidal cross-section allowed for good inference despite the additional complexities in the posterior distribution.


==> priors.tex <==
\section{Priors}
The probability associated with each prior is an open question. The aim is to write priors in such a way that they can be updated as additional information is included. To start, we use simulations to gather our prior information.

We consider imposing priors with Gaussian probabilities. The further our prior argument, f(x), deviates from the expected, $f(x_0)$, the lower the probability. The scale at which this probability reduces is controlled by the prior's uncertainty, $\sigma$. To (reduce subjectivity),  we consider treating this uncertainty as a hyper-parameter in the Bayesian inference.

We consider a prior's argument as $f(\thetavec)$ and the default argument as $f(\thetazerovec)$. Further, the covariance matrix is taken to be $\sigma^2 I_N$. Thus the prior probability, based on the multivariate Gaussian distribution is,
\begin{equation}
    \log(P) = \left(-\frac{1}{2}\sigma^{-2}\left|\left|f(\thetavec)-f(\thetazerovec)\right|\right|^2- \log\left(\sigma\right) - \frac{N}{2}\ln(2\pi) 
 \right)
\end{equation}
To manage (the fact sigma is free and each prior is in different regimes) a series of three transformations are sought. These are designed to remove the impact of N (which depends on the number of grid points), standardise the expected range of the prior's Mahalanobis distance and position the log probability in a range that aligns with the likelihood probabilities in the problem. The resultant log probability is,

\begin{equation}
    \log(P) = A\left(\frac{1}{2}-\frac{1}{2}\sigma^{-2}\frac{\left|\left|f(\thetavec)-f(\thetazerovec)\right|\right|^2}{N \langle (\Delta f)^2 \rangle}- \log\left(\sigma\right) \right)
\end{equation}
The result is such that, were the average difference to the true to be the same as that expected, an uncertainty of 1 results in a log probability of 0. A is a single parameter that needs to be scanned across to find the optimal value. It was found that a value of () was reasonable. This was due to the maximum log probability occurring when 
\begin{equation}
    \sigma_{max} = \frac{\left|\left|f(\thetavec)-f(\thetazerovec)\right|\right|}{\sqrt{N \langle (\Delta f)^2 \rangle}}
\end{equation}
which is to say the variance ought to be the fraction of the solps result. 
This result yields 
\begin{equation}
    \log(P)|_{\sigma_{max}}=-A\log(\sigma_{max}) = -A\left(\log(\left|\left|f(\thetavec)-f(\thetazerovec)\right|\right|) - \frac{1}{2}\log(N \langle (\Delta f)^2 \rangle)\right)
\end{equation}

Therefore the difference in log(P) between a high and low  $\left|\left|f(\thetavec)-f(\thetazerovec)\right|\right|$ is 
\begin{equation}
    \Delta\log(P)|_{\sigma_{max}} = A \log\left(\frac{\left|\left|f(\thetavec)-f(\thetazerovec)\right|\right|_{low }}{\left|\left|f(\thetavec)-f(\thetazerovec)\right|\right|_{high}}\right)
\end{equation}
Half of above?
At low $\left|\left|f(\thetavec)-f(\thetazerovec)\right|\right|$, $\log(P)\to $

Thus if a case has prior argument 25 times worse than the average solps result, it ought to have an uncertainty of 5. This corresponds to a log probability of $\frac{A}{2}\log(\sigma^2)$. Consequently, the difference in probability between choosing solutions at which there is no difference to the true (delta is 0, which has a probability of $\frac{A}{2}\left( 1 - \log(\sigma^2) \right)$ is $A/2$.


